A Low-cost and Portable Active Noise Control Unit

The objective of this research is to employ cutting-edge active noise control methodologies in order to mitigate the noise emissions produced by electrical appliances, such as a coffee machine. The algorithm utilized in this study is the modified Filtered-X Least Mean Square (FXLMS) algorithm. This algorithm aims to generate an anti-noise waveform by utilizing measurements from both the reference microphone and the error microphone. The desired outcome of this approach is to achieve a residual noise level of zero. The primary difficulty lies in conducting the experiment in an open space setting, as conventional active noise control systems are designed to function within enclosed environments, such as closed rooms or relatively confined spaces like the volume inside headphones. A validation test bench is established, employing the Sigma Studio software to oversee the entire system, with the ADAU1452 digital signal processor being chosen. This study presents an introduction to different Active Noise Control systems and algorithms, followed by the execution of simulations for representative techniques. Subsequently, this section provides a comprehensive account of the procedures involved in executing the experiments, followed by an exploration of potential avenues for further research.

==> Front/Graphical_Abstract.tex <==
%=== FRONT PART ===
%=== ABSTRCT ===

%\begin{center}
\chapter*{Graphical Abstract}
\rhead{Graphical Abstract}
%\end{center}
\addcontentsline{toc}{chapter}{Graphical Abstract}
%===============================
% Significance Statement goes here - 100 words limits
%===============================

Proin semper mauris arcu, at sodales dolor lobortis eu. Vestibulum non tempus nibh. Proin id mauris tincidunt, hendrerit ipsum at, placerat lacus. Proin ac malesuada mauris. Ut justo arcu, euismod ac magna sit amet, rutrum gravida sapien. Vestibulum efficitur sodales mattis. Mauris ornare leo nec elit fermentum scelerisque. Nullam nec augue sed ex fringilla sagittis. Suspendisse tincidunt sollicitudin tortor eget vehicula. Sed volutpat scelerisque augue sit amet sodales. Donec eget nisi facilisis, viverra magna ac, cursus purus. Mauris eget augue sit amet lectus tempus lacinia eget eu nisi. Morbi rutrum eros non sapien euismod, id sagittis ipsum sagittis. Phasellus eget.


\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{fig/Graphical-Abstract-example.png}
\end{figure}
%===============================

%=== END OF GRAPHICAL ABSTRACT ===


==> Modified-FXLMS_Experiment/Modified-FXLMS_Experiment.tex <==
\chapter{4. Modified FxLMS Experiments}
\section{Modified FxLMS algorithm physical test in duct (closed environment)}
Due to its high computational efficiency and excellent convergence behavior, the modified FxLMS algorithm has been employed in this part to mitigate the noise present in the duct.  

\subsection{Experimental system setup}
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture21.png}
  \caption{The experimental configuration for the test bench.}
  \label{Fig21}
\end{figure}
%-----------------Figure 2_4----------------------------------

The construction of the test bench is based on the guidelines provided by the official MATLAB website, as shown in Figure~\ref{Fig21}. The subsequent paragraph provides an introduction to the components utilized in the tests and their respective configurations. The elongated cylindrical structure represents the principal conduit, denoting the acoustic component of the adapted FXLMS function block. The system comprises of a noise generator, a reference microphone, and an error microphone. The secondary path refers to a specific branch of the pipe that is equipped with a control source located at its opening. In the conducted experiment, the designated position of the noise source is indicated as 0 cm. The reference microphone is situated at a distance of 8 cm, while the anti-noise source, serving as the initiation point of the secondary path, is positioned at 73 cm. Lastly, the error microphone is put at a distance of 78 cm, representing the termination point of the pipe. The placement of a cotton material behind the reference microphone serves the purpose of preventing the unwanted transmission or interference of the anti-noise signal, hence ensuring the integrity and precision of the reference signal. The software and hardware configuration in SigmaStudio are depicted in Figure~\ref{Fig22} and Figure~\ref{Fig23}, respectively.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture22.png}
  \caption{Sigma Studio hardware connection.}
  \label{Fig22}
\end{figure}
%-----------------Figure 2_4----------------------------------

The hardware configuration involves the connection of an EEProm and an ADAU control unit, facilitating the implementation of real-time active noise reduction. The purpose of EEPROM is to serve as a temporary storage medium for the signal acquired by microphones. In contrast, ADAU1452 is responsible for doing the necessary computations for the updated FxLMS algorithm and supplying the control source with the resulting output signal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture23.png}
  \caption{Sigma Studio software set up.}
  \label{Fig23}
\end{figure}
%-----------------Figure 2_4----------------------------------

The aforementioned software configuration represents a single-channel active noise control (ANC) system. The ADAU1452 chip utilizes two input channels to transmit a reference signal and an error signal to a modified FXLMS function block. This function block incorporates the noise acquired by two microphones.

The modified FXLMS function block is equipped with two distinct operational modes, namely the training mode and the runtime mode. The purpose of the training mode is to calculate the secondary path coefficient, which is then utilized to mitigate the impact of secondary path disturbances. The purpose of the runtime mode is to execute the modified FXLMS algorithm in real-time signal processing. During the training mode, the input for the error signal and the input for the reference signal are both deactivated. Consequently, the signal processing unit exclusively gets the stochastic noise generated at the control source, as well as the ensuing noise captured by the error microphone. The secondary path coefficient can be defined as the ratio between the two signals.

A mute block is implemented at channel 2, specifically at input 16, in order to silence the reference microphone when required. This action is taken, for example, when the training mode is activated or when troubleshooting is necessary. The speaker is connected to channel 1, which represents the anti-noise signal, for the purpose of generating outputs. The additional output is not relevant to the sigma studio project and is deactivated in subsequent experiments.
In order to ascertain the correct connection of the signal and microphones to their respective ports, a preliminary test is undertaken.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture24.png}
  \caption{Channel connection test.}
  \label{Fig24}
\end{figure}
%-----------------Figure 2_4----------------------------------

Loudspeakers and microphones are typically linked to respective output and input pins. In the context of loudspeaker testing, the computer is often linked to the input pin. The accuracy of the connection is determined by the successful production of the intended sound. Microphones are typically linked to computers in order to capture audio signals produced by the computer. When a microphone is properly plugged in, it effectively eliminates any extraneous noise. The validation of the connection between the loudspeakers and the ADAU board has recently been completed. The functionality of this connection may be determined by assessing if the loudspeaker is producing the intended sound. In order to establish proper connections between amplifiers and speakers, it is imperative to exercise care and meticulousness, as both devices possess distinct positive and negative ports that necessitate appropriate interconnections.

\subsection{Experiment process}
The objective of the studies is to determine the optimal settings for the function block, as well as identify the most effective arrangement for the test bench. 

The determination of the filter length, step size, and sampling frequency is required. The determination of the final outcome will be contingent upon the findings obtained from the conducted experiment. The initial phase of the experiment involves training the adaptive filter. Prior to commencing the training process, both input signals are silenced to facilitate the acquisition of the secondary path filter S(z). Once the trained filter has been saved, it can be utilized for testing purposes.

During the training process of the secondary path, the coefficients of the secondary path are trained using three different filter lengths: 32, 64, and 128. The default step size for training is set at 0.9, and the duration of the training session is 30 seconds. The outcomes are stored in a text file for subsequent reference in the run-time mode.

The control variable method is employed during the testing process. The placement of microphones and speakers is predetermined and unalterable. The speaker in the pipe serves as the noise source, emitting a range of noises produced by Audacity. Given that the sampling rate in our specific scenario is 48kHz, and the signal is down-sampled by a factor of 12 before entering the modified FxLMS block, it can be concluded that the effectiveness of the active noise control (ANC) system is limited when it comes to attenuating high frequency noise. However, it was seen that the active noise control (ANC) system was not efficient in attenuating low-frequency noises during the experiment. Consequently, the noise frequencies selected for testing were 250 Hz, 3000 Hz, 400 Hz, 500 Hz, and 600 Hz, as these were the frequencies that could be effectively suppressed by the ANC system. The quantification of noise reduction is determined by comparing the readings obtained from the spectrometer positioned at the terminus of the pipe both prior to and subsequent to the implementation of active noise control. The tables below display the test results obtained under three different situations.

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-5}$}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Frequency}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA) before ANC}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA)  after ANC}} & \multicolumn{1}{c|}{\textbf{NR}} \\ \hline
250hz                                    & 75                                                               & Diverge                                                          & Fail                                          \\ \hline
300hz                                    & 75                                                               & 65                                                               & 10                                            \\ \hline
400hz                                    & 78                                                               & Diverge                                                          & Fail                                          \\ \hline
500hz                                    & 78                                                               & Drop to 72,then Diverge.                                         & Fail                                          \\ \hline
600hz                                    & 76                                                               & 60                                                               & 16                                            \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & Diverge                         & Fail        \\ \hline
300hz              & 75                                    & 53                              & 22          \\ \hline
400hz              & 77                                    & Diverge                         & Fail        \\ \hline
500hz              & 78                                    & 57                              & 21          \\ \hline
600hz              & 76                                    & 60                              & 16          \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 68                              & 7           \\ \hline
300hz              & 77                                    & Diverge                         & Fail        \\ \hline
400hz              & 83                                    & 73                              & 10          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 65                              & 10          \\ \hline
300hz              & 77                                    & Diverge, but very slow.         & Fail        \\ \hline
400hz              & 83                                    & 66                              & 17          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & 74                              & 7           \\ \hline
300hz              & 76                                    & 71                              & 5           \\ \hline
400hz              & 83                                    & 80, but not stable              & 3           \\ \hline
500hz              & 81                                    & 79                              & 2           \\ \hline
600hz              & 83                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & Diverge, but very slow          & Fail        \\ \hline
300hz              & 76                                    & 56                              & 20          \\ \hline
400hz              & 83                                    & 65                              & 18          \\ \hline
500hz              & 81                                    & 64                              & 17          \\ \hline
600hz              & 83                                    & Diverge, but very slow          & Fail        \\ \hline
\end{tabular}
\end{table}

The efficacy of each sort of parameter is demonstrated by constructing histograms that display the outcomes of the filters on lowering noises of frequencies $300$ Hz and $500$ Hz, as depicted in Figure~\ref{Fig25} and Figure~\ref{Fig26}.

%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture25.png}
  \caption{Noise performance at $300$ Hz tonal noise.}
  \label{Fig25}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture26.png}
  \caption{Noise performance at $500$ Hz tonal noise.}
  \label{Fig26}
\end{figure}
%-----------------Figure 2_4----------------------------------
It is evident that increasing the length of the filter leads to improved stability in performance. This is due to the occurrence of random divergence at certain frequencies when using shorter filter lengths. A filter length of $128$ has been chosen, together with a step size of $10^{-6}$, in order to achieve improved noise reduction.

In conclusion, the system is subjected to testing in the presence of broadband noise. This noise is generated by two sources: the first source is white noise produced by Audacity, with a frequency range of $350$ Hz to $450$ Hz. The second source consists of a combination of tonal noise at $300$ Hz and tonal noise at $400$ Hz.

The initial white noise exhibits a loudness range of 65 to 67 dB. However, following the implementation of the modified FXLMS unit, the loudness is effectively decreased to a range of 54 to 56 dB. Additionally, the combination of tonal noises experiences a reduction from 89 dB to 70 dB. Overall, the noise control demonstrates reliable performance. In general, it can be inferred that the current active noise control (ANC) unit demonstrates efficacy across the frequency range of $300$ Hz to approximately $500$ Hz. 

Several potential limits and downsides have been identified and are presented in the following list:
\begin{enumerate}
    \item The noise source fails to generate noise of superior quality, hence impeding our ability to accurately assess the efficacy of the ANC system.
    \item The magnitude of measurement inaccuracy is significant due to the manual handling of the sound meter, which inevitably leads to variations in its position during several experimental trials. It is plausible that the optimal arrangement of components has yet to be achieved.
\end{enumerate}

\section{Modified FxLMS algorithm test in open space}
\subsection{Physical Set-up}
A wooden structure is constructed to accommodate the components, as the outcome of solely providing a single anti-noise source is highly unfavorable. In an attempt to provide a more comprehensive analysis, efforts were made to position the anti-noise speaker at various orientations surrounding the platform. However, no discernible reduction in noise levels was seen. Therefore, the decision has been made to employ a pair of anti-noise sources positioned symmetrically to the noise source, as the outputs of both speakers are identical. In other terms, the objective is to develop a dual-channel active noise control system. Furthermore, as a result of the vibrations generated by the anti-noise speakers, an additional auditory output is produced when the speakers come into contact with the test bench. To mitigate this issue, two wooden stands have been constructed as a precautionary measure. The software logic remains consistent with earlier instances, although the noise source introduces recorded coffee machine noise. The photograph presented in Figure~\ref{Fig27} illustrates the posture that is reasonably ideal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture27.png}
  \caption{Test bench for open space modified FxLMS ANC}
  \label{Fig27}
\end{figure}
%-----------------Figure 2_4----------------------------------

In order to provide additional information, it should be noted that the error microphone is positioned at a distance of approximately 40 cm from the control sources. In the event that a reference microphone is present, it is positioned directly in front of the noise source. Additionally, a technique is introduced wherein the reference signal is directly connected to the computer, which serves as the noise generator. This approach aims to enhance the accuracy of the reference signal.

\subsection{Software set-up}
As demonstrated previously, the quantity of control sources has been augmented to two, necessitating corresponding adjustments within the Sigma studio software. In order to achieve this, the outputs of two anti-noise speakers have been selected to be identical. Consequently, a sound spliter has been connected to the output terminal of the modified FxLMS block. To mitigate measurement inaccuracies and enhance computational efficiency, the noise signal is directly linked to the board via USB, originating from the computer, as opposed to using a reference microphone. The comprehensive project is displayed in Figure~\ref{Fig28}, Figure~\ref{Fig29}, and Figure~\ref{Fig30} below.  
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture28.png}
  \caption{Complete software set up for two control sources modified FxLMS}
  \label{Fig28}
\end{figure}
%-----------------Figure 2_4----------------------------------

The supported function blocks regulate the sampling rate of the incoming data to the modified FxLMS block and the outgoing data to the control sources. The $down-24$ downsampling function and $up-24$ upsampling function are the subject of inquiry.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture29.png}
  \caption{Down sampling function}
  \label{Fig29}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture30.png}
  \caption{Up sampling function}
  \label{Fig30}
\end{figure}
%-----------------Figure 2_4----------------------------------
The overall value of down-sampling or up-sampling (in terms of multiplication) is obtained by multiplying the values of two separate up-sampling and down-sampling processes. Additional low pass filters can be incorporated in order to get higher values. It is anticipated that modifying the sample rate has the potential to enhance noise compression.

\subsection{Experiment process}
The system is designed to address two distinct forms of noise. The first kind is subjected to filtration through a band-pass filter with a permissible frequency range of 300 Hz to 500 Hz. The second type corresponds to the actual noise produced by the coffee machine, and its spectrogram is depicted in Figure~\ref{Fig30}. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture31.png}
  \caption{The spectrogram of coffee machine noise}
  \label{Fig31}
\end{figure}
%-----------------Figure 2_4----------------------------------

The outcome of the preceding section is employed, wherein a modified FxLMS function block with a filter length of 128 and a training step size of $10^{-6}$ is implemented. Different sample rates are examined to determine the system characteristic that can effectively attenuate the widest range of noise frequencies.

The objective of the experimental procedure is to identify an initial system configuration that is approximately optimal. This involves establishing a fixed sampling rate for the program and adjusting the positions of the anti-noise speakers and error microphone. Next, it is necessary to reposition the microphone and speakers, as well as make appropriate adjustments to the sampling rate. Ultimately, the adjustment of the microphone and speakers' placement is necessary in order to complete the system design.

Initially, the sampling rate is set at a fixed value of 6 kHz. The determination of the position and angle of anti-noise sources involves doing numerous trials. Initially, the anti-noise speakers are placed adjacent to the noise source, while the error microphone is positioned at distances of 25 cm, 35cm, and 45cm from it. A noise compression of approximately 3dB occurs when the error microphone is positioned at distances of either 35cm or 45cm from the noise source. Subsequently, the anti-noise speakers are positioned adjacent to the test bench, with a separation of 10 cm, 20 cm, and 30 cm between each speaker and the noise source. The optimal outcome for reducing tone noise by 2dB is achieved when the positions are set at 10cm and 20 cm. Finally, the placement of the anti-noise speakers in opposition to the noise source is found to be impractical, as it aligns with the physical principles of wave propagation.

The results corresponding to the optimal system configuration are presented in Table~\ref{table7}.
\begin{table}[htbp]
\caption{Noise reduction performance of open space ANC system}\label{table7}
\centering
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Sampling rate}} & \multicolumn{1}{l|}{\textbf{Filtered noise}} & \multicolumn{1}{l|}{\textbf{Actual noise}} \\ \hline
48khz/4                                      & 7dB, but the processing is slow.             & 3dB                                        \\ \hline
48khz/8                                      & 6dB                                          & 2$\sim$3dB                                 \\ \hline
48khz/12                                     & 6dB                                          & 1dB                                        \\ \hline
\end{tabular}
\end{table}
The performance of the sampling rate at 12kHz is exceptional; yet, the high sampling rate poses a threat due to its low processing and convergence speed.
Following the fine-tuning process, the anti-noise speakers have been positioned at a set distance of 5cm adjacent to the noise source. Consequently, both the noise wave and the anti-noise wave propagate in a parallel fashion. The error microphone is positioned at a distance of 40 cm in an open space environment. When the error microphone is moved within a radius of around 3cm, its displacement has a minimal impact on the final result.

\subsection{Experiment conclusion}
In summary, the ANC system that has been developed, in conjunction with the adapted FxLMS algorithm, demonstrates the capability to effectively attenuate noise levels in optimal circumstances characterized by minimal disturbances and straightforward sound propagation paths. This is evident in the results obtained from the duct experiment, where the sound propagation direction remains constant and extraneous noises are effectively blocked.

In the context of an open space environment, the system continues to demonstrate its effectiveness in efficiently mitigating the presence of filtered narrowband noise. The observed reduction in noise levels is substantial enough to be perceptible to individuals. Nevertheless, the system exhibits limited proficiency in dealing with unpredictable and fluctuating real-life noises due to the intricate nature of noise and the inherent constraints of the tools employed. The propagation of noise in open space occurs in multiple directions. However, our system is equipped with only one error microphone and two anti-noise speakers. It is possible that the system's performance could be improved by covering a greater range of directions. Additionally, there are hardware limitations that contribute to the system's shortcomings, such as delays in pre-amplifiers and limitations in the processing power of the chip.

The tests conducted aimed to validate the efficacy and underlying processes of the improved FXLMS algorithm. Furthermore, the optimal configurations of function block parameters, as well as the physical layouts of the platform and the test bench, are attained. Finally, suggestions are put forth to enhance the overall system functionality as well as the physical attributes of each individual component.  

==> Modified-FXLMS__Experiment/Modified-FXLMS_Experiment.tex <==
\chapter{4. Modified FxLMS Experiments}
\section{Modified FxLMS algorithm physical test in duct (closed environment)}
Due to its high computational efficiency and excellent convergence behavior, the modified FxLMS algorithm has been employed in this part to mitigate the noise present in the duct.  

\subsection{Experimental system setup}
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture21.png}
  \caption{The experimental configuration for the test bench.}
  \label{Fig21}
\end{figure}
%-----------------Figure 2_4----------------------------------

The construction of the test bench is based on the guidelines provided by the official MATLAB website, as shown in Figure~\ref{Fig21}. The subsequent paragraph provides an introduction to the components utilized in the tests and their respective configurations. The elongated cylindrical structure represents the principal conduit, denoting the acoustic component of the adapted FXLMS function block. The system comprises of a noise generator, a reference microphone, and an error microphone. The secondary path refers to a specific branch of the pipe that is equipped with a control source located at its opening. In the conducted experiment, the designated position of the noise source is indicated as 0 cm. The reference microphone is situated at a distance of 8 cm, while the anti-noise source, serving as the initiation point of the secondary path, is positioned at 73 cm. Lastly, the error microphone is put at a distance of 78 cm, representing the termination point of the pipe. The placement of a cotton material behind the reference microphone serves the purpose of preventing the unwanted transmission or interference of the anti-noise signal, hence ensuring the integrity and precision of the reference signal. The software and hardware configuration in SigmaStudio are depicted in Figure~\ref{Fig22} and Figure~\ref{Fig23}, respectively.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture22.png}
  \caption{Sigma Studio hardware connection.}
  \label{Fig22}
\end{figure}
%-----------------Figure 2_4----------------------------------

The hardware configuration involves the connection of an EEProm and an ADAU control unit, facilitating the implementation of real-time active noise reduction. The purpose of EEPROM is to serve as a temporary storage medium for the signal acquired by microphones. In contrast, ADAU1452 is responsible for doing the necessary computations for the updated FxLMS algorithm and supplying the control source with the resulting output signal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture23.png}
  \caption{Sigma Studio software set up.}
  \label{Fig23}
\end{figure}
%-----------------Figure 2_4----------------------------------

The aforementioned software configuration represents a single-channel active noise control (ANC) system. The ADAU1452 chip utilizes two input channels to transmit a reference signal and an error signal to a modified FXLMS function block. This function block incorporates the noise acquired by two microphones.

The modified FXLMS function block is equipped with two distinct operational modes, namely the training mode and the runtime mode. The purpose of the training mode is to calculate the secondary path coefficient, which is then utilized to mitigate the impact of secondary path disturbances. The purpose of the runtime mode is to execute the modified FXLMS algorithm in real-time signal processing. During the training mode, the input for the error signal and the input for the reference signal are both deactivated. Consequently, the signal processing unit exclusively gets the stochastic noise generated at the control source, as well as the ensuing noise captured by the error microphone. The secondary path coefficient can be defined as the ratio between the two signals.

A mute block is implemented at channel 2, specifically at input 16, in order to silence the reference microphone when required. This action is taken, for example, when the training mode is activated or when troubleshooting is necessary. The speaker is connected to channel 1, which represents the anti-noise signal, for the purpose of generating outputs. The additional output is not relevant to the sigma studio project and is deactivated in subsequent experiments.
In order to ascertain the correct connection of the signal and microphones to their respective ports, a preliminary test is undertaken.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture24.png}
  \caption{Channel connection test.}
  \label{Fig24}
\end{figure}
%-----------------Figure 2_4----------------------------------

Loudspeakers and microphones are typically linked to respective output and input pins. In the context of loudspeaker testing, the computer is often linked to the input pin. The accuracy of the connection is determined by the successful production of the intended sound. Microphones are typically linked to computers in order to capture audio signals produced by the computer. When a microphone is properly plugged in, it effectively eliminates any extraneous noise. The validation of the connection between the loudspeakers and the ADAU board has recently been completed. The functionality of this connection may be determined by assessing if the loudspeaker is producing the intended sound. In order to establish proper connections between amplifiers and speakers, it is imperative to exercise care and meticulousness, as both devices possess distinct positive and negative ports that necessitate appropriate interconnections.

\subsection{Experiment process}
The objective of the studies is to determine the optimal settings for the function block, as well as identify the most effective arrangement for the test bench. 

The determination of the filter length, step size, and sampling frequency is required. The determination of the final outcome will be contingent upon the findings obtained from the conducted experiment. The initial phase of the experiment involves training the adaptive filter. Prior to commencing the training process, both input signals are silenced to facilitate the acquisition of the secondary path filter S(z). Once the trained filter has been saved, it can be utilized for testing purposes.

During the training process of the secondary path, the coefficients of the secondary path are trained using three different filter lengths: 32, 64, and 128. The default step size for training is set at 0.9, and the duration of the training session is 30 seconds. The outcomes are stored in a text file for subsequent reference in the run-time mode.

The control variable method is employed during the testing process. The placement of microphones and speakers is predetermined and unalterable. The speaker in the pipe serves as the noise source, emitting a range of noises produced by Audacity. Given that the sampling rate in our specific scenario is 48kHz, and the signal is down-sampled by a factor of 12 before entering the modified FxLMS block, it can be concluded that the effectiveness of the active noise control (ANC) system is limited when it comes to attenuating high frequency noise. However, it was seen that the active noise control (ANC) system was not efficient in attenuating low-frequency noises during the experiment. Consequently, the noise frequencies selected for testing were 250 Hz, 3000 Hz, 400 Hz, 500 Hz, and 600 Hz, as these were the frequencies that could be effectively suppressed by the ANC system. The quantification of noise reduction is determined by comparing the readings obtained from the spectrometer positioned at the terminus of the pipe both prior to and subsequent to the implementation of active noise control. The tables below display the test results obtained under three different situations.

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-5}$}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Frequency}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA) before ANC}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA)  after ANC}} & \multicolumn{1}{c|}{\textbf{NR}} \\ \hline
250hz                                    & 75                                                               & Diverge                                                          & Fail                                          \\ \hline
300hz                                    & 75                                                               & 65                                                               & 10                                            \\ \hline
400hz                                    & 78                                                               & Diverge                                                          & Fail                                          \\ \hline
500hz                                    & 78                                                               & Drop to 72,then Diverge.                                         & Fail                                          \\ \hline
600hz                                    & 76                                                               & 60                                                               & 16                                            \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & Diverge                         & Fail        \\ \hline
300hz              & 75                                    & 53                              & 22          \\ \hline
400hz              & 77                                    & Diverge                         & Fail        \\ \hline
500hz              & 78                                    & 57                              & 21          \\ \hline
600hz              & 76                                    & 60                              & 16          \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 68                              & 7           \\ \hline
300hz              & 77                                    & Diverge                         & Fail        \\ \hline
400hz              & 83                                    & 73                              & 10          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 65                              & 10          \\ \hline
300hz              & 77                                    & Diverge, but very slow.         & Fail        \\ \hline
400hz              & 83                                    & 66                              & 17          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & 74                              & 7           \\ \hline
300hz              & 76                                    & 71                              & 5           \\ \hline
400hz              & 83                                    & 80, but not stable              & 3           \\ \hline
500hz              & 81                                    & 79                              & 2           \\ \hline
600hz              & 83                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & Diverge, but very slow          & Fail        \\ \hline
300hz              & 76                                    & 56                              & 20          \\ \hline
400hz              & 83                                    & 65                              & 18          \\ \hline
500hz              & 81                                    & 64                              & 17          \\ \hline
600hz              & 83                                    & Diverge, but very slow          & Fail        \\ \hline
\end{tabular}
\end{table}

The efficacy of each sort of parameter is demonstrated by constructing histograms that display the outcomes of the filters on lowering noises of frequencies $300$ Hz and $500$ Hz, as depicted in Figure~\ref{Fig25} and Figure~\ref{Fig26}.

%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture25.png}
  \caption{Noise performance at $300$ Hz tonal noise.}
  \label{Fig25}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture26.png}
  \caption{Noise performance at $500$ Hz tonal noise.}
  \label{Fig26}
\end{figure}
%-----------------Figure 2_4----------------------------------
It is evident that increasing the length of the filter leads to improved stability in performance. This is due to the occurrence of random divergence at certain frequencies when using shorter filter lengths. A filter length of $128$ has been chosen, together with a step size of $10^{-6}$, in order to achieve improved noise reduction.

In conclusion, the system is subjected to testing in the presence of broadband noise. This noise is generated by two sources: the first source is white noise produced by Audacity, with a frequency range of $350$ Hz to $450$ Hz. The second source consists of a combination of tonal noise at $300$ Hz and tonal noise at $400$ Hz.

The initial white noise exhibits a loudness range of 65 to 67 dB. However, following the implementation of the modified FXLMS unit, the loudness is effectively decreased to a range of 54 to 56 dB. Additionally, the combination of tonal noises experiences a reduction from 89 dB to 70 dB. Overall, the noise control demonstrates reliable performance. In general, it can be inferred that the current active noise control (ANC) unit demonstrates efficacy across the frequency range of $300$ Hz to approximately $500$ Hz. 

Several potential limits and downsides have been identified and are presented in the following list:
\begin{enumerate}
    \item The noise source fails to generate noise of superior quality, hence impeding our ability to accurately assess the efficacy of the ANC system.
    \item The magnitude of measurement inaccuracy is significant due to the manual handling of the sound meter, which inevitably leads to variations in its position during several experimental trials. It is plausible that the optimal arrangement of components has yet to be achieved.
\end{enumerate}

\section{Modified FxLMS algorithm test in open space}
\subsection{Physical Set-up}
A wooden structure is constructed to accommodate the components, as the outcome of solely providing a single anti-noise source is highly unfavorable. In an attempt to provide a more comprehensive analysis, efforts were made to position the anti-noise speaker at various orientations surrounding the platform. However, no discernible reduction in noise levels was seen. Therefore, the decision has been made to employ a pair of anti-noise sources positioned symmetrically to the noise source, as the outputs of both speakers are identical. In other terms, the objective is to develop a dual-channel active noise control system. Furthermore, as a result of the vibrations generated by the anti-noise speakers, an additional auditory output is produced when the speakers come into contact with the test bench. To mitigate this issue, two wooden stands have been constructed as a precautionary measure. The software logic remains consistent with earlier instances, although the noise source introduces recorded coffee machine noise. The photograph presented in Figure~\ref{Fig27} illustrates the posture that is reasonably ideal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture27.png}
  \caption{Test bench for open space modified FxLMS ANC}
  \label{Fig27}
\end{figure}
%-----------------Figure 2_4----------------------------------

In order to provide additional information, it should be noted that the error microphone is positioned at a distance of approximately 40 cm from the control sources. In the event that a reference microphone is present, it is positioned directly in front of the noise source. Additionally, a technique is introduced wherein the reference signal is directly connected to the computer, which serves as the noise generator. This approach aims to enhance the accuracy of the reference signal.

\subsection{Software set-up}
As demonstrated previously, the quantity of control sources has been augmented to two, necessitating corresponding adjustments within the Sigma studio software. In order to achieve this, the outputs of two anti-noise speakers have been selected to be identical. Consequently, a sound spliter has been connected to the output terminal of the modified FxLMS block. To mitigate measurement inaccuracies and enhance computational efficiency, the noise signal is directly linked to the board via USB, originating from the computer, as opposed to using a reference microphone. The comprehensive project is displayed in Figure~\ref{Fig28}, Figure~\ref{Fig29}, and Figure~\ref{Fig30} below.  
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture28.png}
  \caption{Complete software set up for two control sources modified FxLMS}
  \label{Fig28}
\end{figure}
%-----------------Figure 2_4----------------------------------

The supported function blocks regulate the sampling rate of the incoming data to the modified FxLMS block and the outgoing data to the control sources. The $down-24$ downsampling function and $up-24$ upsampling function are the subject of inquiry.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture29.png}
  \caption{Down sampling function}
  \label{Fig29}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture30.png}
  \caption{Up sampling function}
  \label{Fig30}
\end{figure}
%-----------------Figure 2_4----------------------------------
The overall value of down-sampling or up-sampling (in terms of multiplication) is obtained by multiplying the values of two separate up-sampling and down-sampling processes. Additional low pass filters can be incorporated in order to get higher values. It is anticipated that modifying the sample rate has the potential to enhance noise compression.

\subsection{Experiment process}
The system is designed to address two distinct forms of noise. The first kind is subjected to filtration through a band-pass filter with a permissible frequency range of 300 Hz to 500 Hz. The second type corresponds to the actual noise produced by the coffee machine, and its spectrogram is depicted in Figure~\ref{Fig30}. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture31.png}
  \caption{The spectrogram of coffee machine noise}
  \label{Fig31}
\end{figure}
%-----------------Figure 2_4----------------------------------

The outcome of the preceding section is employed, wherein a modified FxLMS function block with a filter length of 128 and a training step size of $10^{-6}$ is implemented. Different sample rates are examined to determine the system characteristic that can effectively attenuate the widest range of noise frequencies.

The objective of the experimental procedure is to identify an initial system configuration that is approximately optimal. This involves establishing a fixed sampling rate for the program and adjusting the positions of the anti-noise speakers and error microphone. Next, it is necessary to reposition the microphone and speakers, as well as make appropriate adjustments to the sampling rate. Ultimately, the adjustment of the microphone and speakers' placement is necessary in order to complete the system design.

Initially, the sampling rate is set at a fixed value of 6 kHz. The determination of the position and angle of anti-noise sources involves doing numerous trials. Initially, the anti-noise speakers are placed adjacent to the noise source, while the error microphone is positioned at distances of 25 cm, 35cm, and 45cm from it. A noise compression of approximately 3dB occurs when the error microphone is positioned at distances of either 35cm or 45cm from the noise source. Subsequently, the anti-noise speakers are positioned adjacent to the test bench, with a separation of 10 cm, 20 cm, and 30 cm between each speaker and the noise source. The optimal outcome for reducing tone noise by 2dB is achieved when the positions are set at 10cm and 20 cm. Finally, the placement of the anti-noise speakers in opposition to the noise source is found to be impractical, as it aligns with the physical principles of wave propagation.

The results corresponding to the optimal system configuration are presented in Table~\ref{table7}.
\begin{table}[htbp]
\caption{Noise reduction performance of open space ANC system}\label{table7}
\centering
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Sampling rate}} & \multicolumn{1}{l|}{\textbf{Filtered noise}} & \multicolumn{1}{l|}{\textbf{Actual noise}} \\ \hline
48khz/4                                      & 7dB, but the processing is slow.             & 3dB                                        \\ \hline
48khz/8                                      & 6dB                                          & 2$\sim$3dB                                 \\ \hline
48khz/12                                     & 6dB                                          & 1dB                                        \\ \hline
\end{tabular}
\end{table}
The performance of the sampling rate at 12kHz is exceptional; yet, the high sampling rate poses a threat due to its low processing and convergence speed.
Following the fine-tuning process, the anti-noise speakers have been positioned at a set distance of 5cm adjacent to the noise source. Consequently, both the noise wave and the anti-noise wave propagate in a parallel fashion. The error microphone is positioned at a distance of 40 cm in an open space environment. When the error microphone is moved within a radius of around 3cm, its displacement has a minimal impact on the final result.

\subsection{Experiment conclusion}
In summary, the ANC system that has been developed, in conjunction with the adapted FxLMS algorithm, demonstrates the capability to effectively attenuate noise levels in optimal circumstances characterized by minimal disturbances and straightforward sound propagation paths. This is evident in the results obtained from the duct experiment, where the sound propagation direction remains constant and extraneous noises are effectively blocked.

In the context of an open space environment, the system continues to demonstrate its effectiveness in efficiently mitigating the presence of filtered narrowband noise. The observed reduction in noise levels is substantial enough to be perceptible to individuals. Nevertheless, the system exhibits limited proficiency in dealing with unpredictable and fluctuating real-life noises due to the intricate nature of noise and the inherent constraints of the tools employed. The propagation of noise in open space occurs in multiple directions. However, our system is equipped with only one error microphone and two anti-noise speakers. It is possible that the system's performance could be improved by covering a greater range of directions. Additionally, there are hardware limitations that contribute to the system's shortcomings, such as delays in pre-amplifiers and limitations in the processing power of the chip.

The tests conducted aimed to validate the efficacy and underlying processes of the improved FXLMS algorithm. Furthermore, the optimal configurations of function block parameters, as well as the physical layouts of the platform and the test bench, are attained. Finally, suggestions are put forth to enhance the overall system functionality as well as the physical attributes of each individual component.  

==> Modified_FXLMS__Experiment/Modified-FXLMS_Experiment.tex <==
\chapter{4. Modified FxLMS Experiments}
\section{Modified FxLMS algorithm physical test in duct (closed environment)}
Due to its high computational efficiency and excellent convergence behavior, the modified FxLMS algorithm has been employed in this part to mitigate the noise present in the duct.  

\subsection{Experimental system setup}
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture21.png}
  \caption{The experimental configuration for the test bench.}
  \label{Fig21}
\end{figure}
%-----------------Figure 2_4----------------------------------

The construction of the test bench is based on the guidelines provided by the official MATLAB website, as shown in Figure~\ref{Fig21}. The subsequent paragraph provides an introduction to the components utilized in the tests and their respective configurations. The elongated cylindrical structure represents the principal conduit, denoting the acoustic component of the adapted FXLMS function block. The system comprises of a noise generator, a reference microphone, and an error microphone. The secondary path refers to a specific branch of the pipe that is equipped with a control source located at its opening. In the conducted experiment, the designated position of the noise source is indicated as 0 cm. The reference microphone is situated at a distance of 8 cm, while the anti-noise source, serving as the initiation point of the secondary path, is positioned at 73 cm. Lastly, the error microphone is put at a distance of 78 cm, representing the termination point of the pipe. The placement of a cotton material behind the reference microphone serves the purpose of preventing the unwanted transmission or interference of the anti-noise signal, hence ensuring the integrity and precision of the reference signal. The software and hardware configuration in SigmaStudio are depicted in Figure~\ref{Fig22} and Figure~\ref{Fig23}, respectively.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=14cm]{fig/Picture22.png}
  \caption{Sigma Studio hardware connection.}
  \label{Fig22}
\end{figure}
%-----------------Figure 2_4----------------------------------

The hardware configuration involves the connection of an EEProm and an ADAU control unit, facilitating the implementation of real-time active noise reduction. The purpose of EEPROM is to serve as a temporary storage medium for the signal acquired by microphones. In contrast, ADAU1452 is responsible for doing the necessary computations for the updated FxLMS algorithm and supplying the control source with the resulting output signal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture23.png}
  \caption{Sigma Studio software set up.}
  \label{Fig23}
\end{figure}
%-----------------Figure 2_4----------------------------------

The aforementioned software configuration represents a single-channel active noise control (ANC) system. The ADAU1452 chip utilizes two input channels to transmit a reference signal and an error signal to a modified FXLMS function block. This function block incorporates the noise acquired by two microphones.

The modified FXLMS function block is equipped with two distinct operational modes, namely the training mode and the runtime mode. The purpose of the training mode is to calculate the secondary path coefficient, which is then utilized to mitigate the impact of secondary path disturbances. The purpose of the runtime mode is to execute the modified FXLMS algorithm in real-time signal processing. During the training mode, the input for the error signal and the input for the reference signal are both deactivated. Consequently, the signal processing unit exclusively gets the stochastic noise generated at the control source, as well as the ensuing noise captured by the error microphone. The secondary path coefficient can be defined as the ratio between the two signals.

A mute block is implemented at channel 2, specifically at input 16, in order to silence the reference microphone when required. This action is taken, for example, when the training mode is activated or when troubleshooting is necessary. The speaker is connected to channel 1, which represents the anti-noise signal, for the purpose of generating outputs. The additional output is not relevant to the sigma studio project and is deactivated in subsequent experiments.
In order to ascertain the correct connection of the signal and microphones to their respective ports, a preliminary test is undertaken.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture24.png}
  \caption{Channel connection test.}
  \label{Fig24}
\end{figure}
%-----------------Figure 2_4----------------------------------

Loudspeakers and microphones are typically linked to respective output and input pins. In the context of loudspeaker testing, the computer is often linked to the input pin. The accuracy of the connection is determined by the successful production of the intended sound. Microphones are typically linked to computers in order to capture audio signals produced by the computer. When a microphone is properly plugged in, it effectively eliminates any extraneous noise. The validation of the connection between the loudspeakers and the ADAU board has recently been completed. The functionality of this connection may be determined by assessing if the loudspeaker is producing the intended sound. In order to establish proper connections between amplifiers and speakers, it is imperative to exercise care and meticulousness, as both devices possess distinct positive and negative ports that necessitate appropriate interconnections.

\subsection{Experiment process}
The objective of the studies is to determine the optimal settings for the function block, as well as identify the most effective arrangement for the test bench. 

The determination of the filter length, step size, and sampling frequency is required. The determination of the final outcome will be contingent upon the findings obtained from the conducted experiment. The initial phase of the experiment involves training the adaptive filter. Prior to commencing the training process, both input signals are silenced to facilitate the acquisition of the secondary path filter S(z). Once the trained filter has been saved, it can be utilized for testing purposes.

During the training process of the secondary path, the coefficients of the secondary path are trained using three different filter lengths: 32, 64, and 128. The default step size for training is set at 0.9, and the duration of the training session is 30 seconds. The outcomes are stored in a text file for subsequent reference in the run-time mode.

The control variable method is employed during the testing process. The placement of microphones and speakers is predetermined and unalterable. The speaker in the pipe serves as the noise source, emitting a range of noises produced by Audacity. Given that the sampling rate in our specific scenario is 48kHz, and the signal is down-sampled by a factor of 12 before entering the modified FxLMS block, it can be concluded that the effectiveness of the active noise control (ANC) system is limited when it comes to attenuating high frequency noise. However, it was seen that the active noise control (ANC) system was not efficient in attenuating low-frequency noises during the experiment. Consequently, the noise frequencies selected for testing were 250 Hz, 3000 Hz, 400 Hz, 500 Hz, and 600 Hz, as these were the frequencies that could be effectively suppressed by the ANC system. The quantification of noise reduction is determined by comparing the readings obtained from the spectrometer positioned at the terminus of the pipe both prior to and subsequent to the implementation of active noise control. The tables below display the test results obtained under three different situations.

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-5}$}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Frequency}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA) before ANC}} & \multicolumn{1}{c|}{\textbf{Noise level (dBA)  after ANC}} & \multicolumn{1}{c|}{\textbf{NR}} \\ \hline
250hz                                    & 75                                                               & Diverge                                                          & Fail                                          \\ \hline
300hz                                    & 75                                                               & 65                                                               & 10                                            \\ \hline
400hz                                    & 78                                                               & Diverge                                                          & Fail                                          \\ \hline
500hz                                    & 78                                                               & Drop to 72,then Diverge.                                         & Fail                                          \\ \hline
600hz                                    & 76                                                               & 60                                                               & 16                                            \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $32$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & Diverge                         & Fail        \\ \hline
300hz              & 75                                    & 53                              & 22          \\ \hline
400hz              & 77                                    & Diverge                         & Fail        \\ \hline
500hz              & 78                                    & 57                              & 21          \\ \hline
600hz              & 76                                    & 60                              & 16          \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 68                              & 7           \\ \hline
300hz              & 77                                    & Diverge                         & Fail        \\ \hline
400hz              & 83                                    & 73                              & 10          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $64$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 75                                    & 65                              & 10          \\ \hline
300hz              & 77                                    & Diverge, but very slow.         & Fail        \\ \hline
400hz              & 83                                    & 66                              & 17          \\ \hline
500hz              & 82                                    & Diverge                         & Fail        \\ \hline
600hz              & 84                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-5}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & 74                              & 7           \\ \hline
300hz              & 76                                    & 71                              & 5           \\ \hline
400hz              & 83                                    & 80, but not stable              & 3           \\ \hline
500hz              & 81                                    & 79                              & 2           \\ \hline
600hz              & 83                                    & Diverge                         & Fail        \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Filter length: $128$, step size: $10^{-6}$}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Frequency} & \textbf{Noise level (dBA) before ANC} & \textbf{Noise level (dBA)  ANC} & \textbf{NR} \\ \hline
250hz              & 81                                    & Diverge, but very slow          & Fail        \\ \hline
300hz              & 76                                    & 56                              & 20          \\ \hline
400hz              & 83                                    & 65                              & 18          \\ \hline
500hz              & 81                                    & 64                              & 17          \\ \hline
600hz              & 83                                    & Diverge, but very slow          & Fail        \\ \hline
\end{tabular}
\end{table}

The efficacy of each sort of parameter is demonstrated by constructing histograms that display the outcomes of the filters on lowering noises of frequencies $300$ Hz and $500$ Hz, as depicted in Figure~\ref{Fig25} and Figure~\ref{Fig26}.

%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture25.png}
  \caption{Noise performance at $300$ Hz tonal noise.}
  \label{Fig25}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=11cm]{fig/Picture26.png}
  \caption{Noise performance at $500$ Hz tonal noise.}
  \label{Fig26}
\end{figure}
%-----------------Figure 2_4----------------------------------
It is evident that increasing the length of the filter leads to improved stability in performance. This is due to the occurrence of random divergence at certain frequencies when using shorter filter lengths. A filter length of $128$ has been chosen, together with a step size of $10^{-6}$, in order to achieve improved noise reduction.

In conclusion, the system is subjected to testing in the presence of broadband noise. This noise is generated by two sources: the first source is white noise produced by Audacity, with a frequency range of $350$ Hz to $450$ Hz. The second source consists of a combination of tonal noise at $300$ Hz and tonal noise at $400$ Hz.

The initial white noise exhibits a loudness range of 65 to 67 dB. However, following the implementation of the modified FXLMS unit, the loudness is effectively decreased to a range of 54 to 56 dB. Additionally, the combination of tonal noises experiences a reduction from 89 dB to 70 dB. Overall, the noise control demonstrates reliable performance. In general, it can be inferred that the current active noise control (ANC) unit demonstrates efficacy across the frequency range of $300$ Hz to approximately $500$ Hz. 

Several potential limits and downsides have been identified and are presented in the following list:
\begin{enumerate}
    \item The noise source fails to generate noise of superior quality, hence impeding our ability to accurately assess the efficacy of the ANC system.
    \item The magnitude of measurement inaccuracy is significant due to the manual handling of the sound meter, which inevitably leads to variations in its position during several experimental trials. It is plausible that the optimal arrangement of components has yet to be achieved.
\end{enumerate}

\section{Modified FxLMS algorithm test in open space}
\subsection{Physical Set-up}
A wooden structure is constructed to accommodate the components, as the outcome of solely providing a single anti-noise source is highly unfavorable. In an attempt to provide a more comprehensive analysis, efforts were made to position the anti-noise speaker at various orientations surrounding the platform. However, no discernible reduction in noise levels was seen. Therefore, the decision has been made to employ a pair of anti-noise sources positioned symmetrically to the noise source, as the outputs of both speakers are identical. In other terms, the objective is to develop a dual-channel active noise control system. Furthermore, as a result of the vibrations generated by the anti-noise speakers, an additional auditory output is produced when the speakers come into contact with the test bench. To mitigate this issue, two wooden stands have been constructed as a precautionary measure. The software logic remains consistent with earlier instances, although the noise source introduces recorded coffee machine noise. The photograph presented in Figure~\ref{Fig27} illustrates the posture that is reasonably ideal. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture27.png}
  \caption{Test bench for open space modified FxLMS ANC}
  \label{Fig27}
\end{figure}
%-----------------Figure 2_4----------------------------------

In order to provide additional information, it should be noted that the error microphone is positioned at a distance of approximately 40 cm from the control sources. In the event that a reference microphone is present, it is positioned directly in front of the noise source. Additionally, a technique is introduced wherein the reference signal is directly connected to the computer, which serves as the noise generator. This approach aims to enhance the accuracy of the reference signal.

\subsection{Software set-up}
As demonstrated previously, the quantity of control sources has been augmented to two, necessitating corresponding adjustments within the Sigma studio software. In order to achieve this, the outputs of two anti-noise speakers have been selected to be identical. Consequently, a sound spliter has been connected to the output terminal of the modified FxLMS block. To mitigate measurement inaccuracies and enhance computational efficiency, the noise signal is directly linked to the board via USB, originating from the computer, as opposed to using a reference microphone. The comprehensive project is displayed in Figure~\ref{Fig28}, Figure~\ref{Fig29}, and Figure~\ref{Fig30} below.  
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture28.png}
  \caption{Complete software set up for two control sources modified FxLMS}
  \label{Fig28}
\end{figure}
%-----------------Figure 2_4----------------------------------

The supported function blocks regulate the sampling rate of the incoming data to the modified FxLMS block and the outgoing data to the control sources. The $down-24$ downsampling function and $up-24$ upsampling function are the subject of inquiry.
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture29.png}
  \caption{Down sampling function}
  \label{Fig29}
\end{figure}
%-----------------Figure 2_4----------------------------------
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture30.png}
  \caption{Up sampling function}
  \label{Fig30}
\end{figure}
%-----------------Figure 2_4----------------------------------
The overall value of down-sampling or up-sampling (in terms of multiplication) is obtained by multiplying the values of two separate up-sampling and down-sampling processes. Additional low pass filters can be incorporated in order to get higher values. It is anticipated that modifying the sample rate has the potential to enhance noise compression.

\subsection{Experiment process}
The system is designed to address two distinct forms of noise. The first kind is subjected to filtration through a band-pass filter with a permissible frequency range of 300 Hz to 500 Hz. The second type corresponds to the actual noise produced by the coffee machine, and its spectrogram is depicted in Figure~\ref{Fig30}. 
%-----------------Figure 2_4----------------------------------
\begin{figure}[htbp]
  \centering
    \includegraphics[width=13cm]{fig/Picture31.png}
  \caption{The spectrogram of coffee machine noise}
  \label{Fig31}
\end{figure}
%-----------------Figure 2_4----------------------------------

The outcome of the preceding section is employed, wherein a modified FxLMS function block with a filter length of 128 and a training step size of $10^{-6}$ is implemented. Different sample rates are examined to determine the system characteristic that can effectively attenuate the widest range of noise frequencies.

The objective of the experimental procedure is to identify an initial system configuration that is approximately optimal. This involves establishing a fixed sampling rate for the program and adjusting the positions of the anti-noise speakers and error microphone. Next, it is necessary to reposition the microphone and speakers, as well as make appropriate adjustments to the sampling rate. Ultimately, the adjustment of the microphone and speakers' placement is necessary in order to complete the system design.

Initially, the sampling rate is set at a fixed value of 6 kHz. The determination of the position and angle of anti-noise sources involves doing numerous trials. Initially, the anti-noise speakers are placed adjacent to the noise source, while the error microphone is positioned at distances of 25 cm, 35cm, and 45cm from it. A noise compression of approximately 3dB occurs when the error microphone is positioned at distances of either 35cm or 45cm from the noise source. Subsequently, the anti-noise speakers are positioned adjacent to the test bench, with a separation of 10 cm, 20 cm, and 30 cm between each speaker and the noise source. The optimal outcome for reducing tone noise by 2dB is achieved when the positions are set at 10cm and 20 cm. Finally, the placement of the anti-noise speakers in opposition to the noise source is found to be impractical, as it aligns with the physical principles of wave propagation.

The results corresponding to the optimal system configuration are presented in Table~\ref{table7}.
\begin{table}[htbp]
\caption{Noise reduction performance of open space ANC system}\label{table7}
\centering
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Sampling rate}} & \multicolumn{1}{l|}{\textbf{Filtered noise}} & \multicolumn{1}{l|}{\textbf{Actual noise}} \\ \hline
48khz/4                                      & 7dB, but the processing is slow.             & 3dB                                        \\ \hline
48khz/8                                      & 6dB                                          & 2$\sim$3dB                                 \\ \hline
48khz/12                                     & 6dB                                          & 1dB                                        \\ \hline
\end{tabular}
\end{table}
The performance of the sampling rate at 12kHz is exceptional; yet, the high sampling rate poses a threat due to its low processing and convergence speed.
Following the fine-tuning process, the anti-noise speakers have been positioned at a set distance of 5cm adjacent to the noise source. Consequently, both the noise wave and the anti-noise wave propagate in a parallel fashion. The error microphone is positioned at a distance of 40 cm in an open space environment. When the error microphone is moved within a radius of around 3cm, its displacement has a minimal impact on the final result.

\subsection{Experiment conclusion}
In summary, the ANC system that has been developed, in conjunction with the adapted FxLMS algorithm, demonstrates the capability to effectively attenuate noise levels in optimal circumstances characterized by minimal disturbances and straightforward sound propagation paths. This is evident in the results obtained from the duct experiment, where the sound propagation direction remains constant and extraneous noises are effectively blocked.

In the context of an open space environment, the system continues to demonstrate its effectiveness in efficiently mitigating the presence of filtered narrowband noise. The observed reduction in noise levels is substantial enough to be perceptible to individuals. Nevertheless, the system exhibits limited proficiency in dealing with unpredictable and fluctuating real-life noises due to the intricate nature of noise and the inherent constraints of the tools employed. The propagation of noise in open space occurs in multiple directions. However, our system is equipped with only one error microphone and two anti-noise speakers. It is possible that the system's performance could be improved by covering a greater range of directions. Additionally, there are hardware limitations that contribute to the system's shortcomings, such as delays in pre-amplifiers and limitations in the processing power of the chip.

The tests conducted aimed to validate the efficacy and underlying processes of the improved FXLMS algorithm. Furthermore, the optimal configurations of function block parameters, as well as the physical layouts of the platform and the test bench, are attained. Finally, suggestions are put forth to enhance the overall system functionality as well as the physical attributes of each individual component.  

==> Results_and_Discussion/Results_and_Discussion.tex <==
%=== Results_and_Discussion ===
%=== (Actual work done and contribution, including literature survey) ===

\chapter{3. Results and Discussion}

\section{Main Activity}

A crucial part of an Android application comprises of `activities'. A set of transcript evaluation were assumed in this project and are summarized at Table \ref{tab:transcript} 

Table \ref{tab:summary2} shows the summary of the performance for each algorithm by acoustic environment (Env.) and the average runtimes (Rt.) for two-source separation. 

\begin{table}[!htp]
    \scriptsize
    \centering
    \begin{tabularx}{\textwidth}{llrlRRRRRR}
\toprule
&Algorithm& 
        Rt. (s) &
                Env. &
                        SDR&    SIR&    SAR&    STOI &  ESTOI & WER\\ \midrule
\multirow{9}{*}{\makecell[cl]{\rotatebox{90}{Raw}}}
&\multirow{3}{*}{\makecell[cl]{AuxIVA}} &
\multirow{3}{*}{358.2}&
LTH &7.218    &8.883    &\textbf{13.310}    &0.675    &0.503    &0.392\\
&&&OFC    &\textbf{8.240}    &10.302    &\textbf{13.316}    &0.705    &0.544    &0.310\\
&&&OTD    &\textbf{14.357}    &17.246    &\textbf{18.263}    &0.780    &0.611    &0.161\\
\cline{2-10}
&\multirow{3}{*}{FastICA} &
\multirow{3}{*}{135.2}&
LTH &\textbf{9.564}    &\textbf{15.960}    &10.961    &0.778    &\textbf{0.609}    &\textbf{0.155}\\
&&&OFC    &7.873    &\textbf{13.206}    &10.001    &\textbf{0.760}    &\textbf{0.599}    &\textbf{0.207}\\
&&&OTD    &10.421    &\textbf{18.700}    &11.281    &0.781    &0.615    &\textbf{0.146}\\
\cline{2-10}
&\multirow{3}{*}{SCA-DSF} &
\multirow{3}{*}{\textbf{96.1}}&
LTH    &9.425    &15.675    &10.917    &\textbf{0.779}    &0.606    &0.167\\
&&&OFC    &7.300    &12.221    &9.805    &0.754    &0.595    &0.224\\
&&&OTD    &9.705    &17.472    &10.852    &\textbf{0.785}    &\textbf{0.622}    &0.162\\
\midrule
\multirow{9}{*}{\makecell[cl]{\rotatebox{90}{Improvement}}}
&\multirow{3}{*}{\makecell[cl]{AuxIVA}} &&
LTH    &16.959    &8.838    &19.726    &0.423    &0.330    &-0.587\\
&&&OFC    &16.471    &10.258    &16.212    &0.394    &0.315    &-0.690\\
&&&OTD    &23.727    &17.041    &24.701    &0.483    &0.440    &-0.820\\
\cline{2-10}
&\multirow{3}{*}{FastICA} &&
LTH    &19.304    &15.915    &17.377    &0.527    &0.436    &-0.824\\
&&&OFC    &16.104    &13.161    &12.897    &0.448    &0.370    &-0.793\\
&&&OTD    &19.791    &18.495    &17.719    &0.484    &0.444    &-0.836\\
\cline{2-10}
&\multirow{3}{*}{SCA-DSF} &&
LTH    &19.166    &15.630    &17.333    &0.528    &0.433    &-0.812\\
&&&OFC    &15.530    &12.176    &12.700    &0.442    &0.365    &-0.776\\
&&&OTD    &19.075    &17.267    &17.290    &0.488    &0.451    &-0.819\\
\midrule
\multicolumn{3}{c}{\multirow{3}{*}{\textit{Input Mixture}}} &
LTH    &-9.741    &0.045    &-6.416    &0.251    &0.173    &0.979\\
&&&OFC    &-8.231    &0.045    &-2.895    &0.311    &0.229    &1.000\\
&&&OTD    &-9.370    &0.205    &-6.438    &0.297    &0.171    &0.982\\
\bottomrule
    \end{tabularx}
    \caption[Performance summary for two-source separation]{Performance summary for two-source separation\\
    {\footnotesize LTH - lecture theatre; OFC - office; OTD - outdoor.}}
    \label{tab:summary2}
\end{table}

The permissions to perform any process with such functionalities must be declared in the manifest as shown in Figure \ref{fig:manifest}.
\begin{figure}[!htb]
    \centering
    \begin{lstlisting}[language=XML]
<?xml version="1.0" encoding="utf-8"?>
<manifest xmlns:android="http://schemas.android.com/apk/res/android"
    <!-- Package declaration...  -->

    <uses-permission android:name="android.permission.RECORD_AUDIO" />
    <uses-permission android:name="android.permission.WRITE_EXTERNAL_STORAGE" />
    <uses-permission android:name="android.permission.INTERNET" />
    <uses-permission android:name="android.permission.ACCESS_NETWORK_STATE" />

    <!-- The rest of the manifest... -->
</manifest>
    \end{lstlisting}
    \caption{Declaration of the permissions required in the Android manifest}
    \label{fig:manifest}
\end{figure}

\FloatBarrier %stopping float objects like images 

\subsection{Recording of the Observed Mixture}
As the user presses the record button (A), the method \texttt{startRecording()} is invoked and the record button's icon changes to a stop symbol as shown in Figure \ref{fig:recordstop}. 
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\textwidth]{fig/recordstop.png}
    \caption{Record button icon changes from a microphone to a stop symbol}
    \label{fig:recordstop}
\end{figure}



%=== END OF RESULTS AND DISCUSSION ===
\newpage

